Variable Packet-Error Coding

We consider a problem in which a source is encoded into N packets, an unknown number of which are subject to adversarial errors en route to the decoder. We seek code designs for which the decoder is guaranteed to be able to reproduce the source subject to a certain distortion constraint when there are no packets errors, subject to a less stringent distortion constraint when there is one error, etc. Focusing on the special case of the erasure distortion measure, we introduce a code design based on the polytope codes of Kosut, Tong, and Tse. The resulting designs are also applied to a separate problem in distributed storage.

==> conclusion.tex <==
The general problem posed in the introduction is akin to the 
multiple-descriptions 
(MD) problem in network information theory~\cite{7}. The difference is
that in the MD problem, packets are either lost or received correctly.
Here they are subject to adversarial errors. This difference seems
to change the problem substantially; polytope codes do not seem to
be useful in the MD problem, for instance. Beyond strengthening
the results provided here, it would be interesting to study a
combination of the two problems in which packets can be either
lost or adversarially changed.

